SAP-DETR: Bridging the Gap Between Salient Points and Queries-Based Transformer Detector for Fast Model Convergency

Recently, the dominant DETR-based approaches apply central-concept spatial prior to accelerate Transformer detector convergency. These methods gradually refine the reference points to the center of target objects and imbue object queries with the updated central reference information for spatially conditional attention. However, centralizing reference points may severely deteriorate queries' saliency and confuse detectors due to the indiscriminative spatial prior. To bridge the gap between the reference points of salient queries and Transformer detectors, we propose SAlient Point-based DETR (SAP-DETR) by treating object detection as a transformation from salient points to instance objects. In SAP-DETR, we explicitly initialize a query-specific reference point for each object query, gradually aggregate them into an instance object, and then predict the distance from each side of the bounding box to these points. By rapidly attending to query-specific reference region and other conditional extreme regions from the image features, SAP-DETR can effectively bridge the gap between the salient point and the query-based Transformer detector with a significant convergency speed. Our extensive experiments have demonstrated that SAP-DETR achieves 1.4 times convergency speed with competitive performance. Under the standard training scheme, SAP-DETR stably promotes the SOTA approaches by 1.0 AP. Based on ResNet-DC-101, SAP-DETR achieves 46.9 AP.

==> SAP-DETR Camera Ready/configuration.tex <==
\begin{table}[t]
  \centering
  \vspace{0.2cm}
  \setlength \tabcolsep{5pt}
    \begin{spacing}{0.85}
    \resizebox{0.491\linewidth}{!}{%
    \begin{tabular}{lc}
    \toprule
    Item  & Value \\
    \midrule
    lr    & 1e-4\\
    lr\_backbone & 1e-5 \\
    weight\_decay & 1e-4 \\
    k\_pe\_temp & 20 \\ 
    q\_point\_pe\_temp & 20 \\
    q\_bbox\_pe\_temp & 20 \\
    enc\_layers & 3 / 6 \\
    dec\_layers & 3 / 6   \\
    dim\_feedforward \hspace{0.66cm} & 2048  \\
    hidden\_dim & 256   \\
    dropout & 0.0  \\
    nheads & 8  \\
    warm\_up & 1000\\
    batch\_size & 4$\times$4 \\
    \specialrule{0pt}{1pt}{1pt}
    \bottomrule
    \end{tabular}}
    \resizebox{0.491\linewidth}{!}{%
    \begin{tabular}{lc}
    \toprule
    Item  & Value \\
    \midrule
    mask\_loss & 1 \\
    obj\_loss & 1 \\
    class\_loss & 1 \\
    bbox\_loss & 5 \\ 
    giou\_loss & 2 \\
    obj\_cost & 2 \\
    class\_cost & 2 \\
    class\_cost & 2 \\
    bbox\_cost & 5 \\
    giou\_cost & 2 \\
    inner\_cost & 9999 \\
    focal\_alpha & 0.25 \\
    transformer\_activation & relu \\
    num\_queries & 400 \\
    \specialrule{0pt}{1pt}{1pt}
    \bottomrule
    \end{tabular}}
    \end{spacing}
    \caption{All configurations of SAP-DETR}
    \label{tab:configuration}%
\end{table}%


==> SAP-DETR Camera Ready/diffhead.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet4'

\begin{table*}[t]
  \centering
   \setlength \tabcolsep{12pt}
    \begin{spacing}{0.7}
    \resizebox{0.78\linewidth}{!}{%
    \begin{tabular}{ccccccccc}
    \toprule
    \multirow{2}[2]{*}{Detach}&\multicolumn{2}{c}{Indep. Prediction Head } & \multicolumn{1}{c}{\multirow{2}[2]{*}{AP}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{AP$_\text{50}$}}& \multicolumn{1}{c}{\multirow{2}[2]{*}{AP$_\text{75}$}}& \multicolumn{1}{c}{\multirow{2}[2]{*}{AP$_\text{S}$}} & 
    \multicolumn{1}{c}{\multirow{2}[2]{*}{AP$_\text{M}$}} &
    \multicolumn{1}{c}{\multirow{2}[2]{*}{AP$_\text{L}$}} \\
    \cmidrule{2-3}  
    &\quad Head$_{\text{cls}}$ & Head$_{\text{bbox}}$  &&&       &       & & \\
    \toprule
    \ding{55}&             &                  &     34.6      & 54.8 & 35.7 & 14.4 & 37.6 & 52.8 \\
    \ding{55}&   \checkmark&                  &     34.7      & 54.8 & 36.0 & \textbf{16.2} & 37.6 &  53.2 \\
    \ding{55}&             &   \checkmark     &     34.8      & 55.0 & 35.8 & 15.3 & 37.8 & 53.5 \\
    \ding{55}&   \checkmark&    \checkmark    &     34.7      & 54.8 & 36.1 & 14.5 & 38.1 & 52.7 \\
    \specialrule{0.5pt}{0.7pt}{1.5pt}
    \checkmark&            &                  &     35.0      & 55.1 & 36.5 & 15.6 & 38.3 & 53.0 \\
    \checkmark& \checkmark &                  &     34.6      & 55.1 & 35.9 & 14.6 & 37.9 & 52.1 \\
    \checkmark&            & \checkmark       & \textbf{35.2} & \textbf{55.4} & \textbf{36.8} & 15.8 &  \textbf{38.5} &  53.6 \\
    \checkmark& \checkmark &  \checkmark      &     35.0      & 55.2 & 36.3 & 14.7 & 38.2 & \textbf{54.0} \\
    \bottomrule
    \end{tabular}}
  \end{spacing}
  \caption{Ablation study on the independent prediction head.}
  \label{tab:diffhead}%
\end{table*}%


==> SAP-DETR Camera Ready/sacling_consistency.tex <==
\begin{table*}[t]
  \centering
   \setlength \tabcolsep{10pt}
    \begin{spacing}{0.7}
    \resizebox{0.78\linewidth}{!}{%
    \begin{tabular}{cccccccccc}
    \toprule
    \multirow{2}[2]{*}{\makecell[c]{Concatenate \\ Box Side PE}}&\multicolumn{3}{c}{Temperature of PE} & \multicolumn{1}{c}{\multirow{2}[2]{*}{AP}} &\multicolumn{1}{c}{\multirow{2}[2]{*}{AP$_\text{50}$}} &\multicolumn{1}{c}{\multirow{2}[2]{*}{AP$_\text{75}$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{AP$_\text{S}$}} & 
    \multicolumn{1}{c}{\multirow{2}[2]{*}{AP$_\text{M}$}} &
    \multicolumn{1}{c}{\multirow{2}[2]{*}{AP$_\text{L}$}} \\
    \cmidrule{2-4}  
    &$T_k$ & $T_{qp}$ & $T_{qb}$ &       &       & & \\
    \toprule
    \ding{55}&         $20$  &     $1000$&   -         & 31.8 & 52.8 & 32.1 & 12.8 & 34.4 & 50.5 \\
    \ding{55}&        $1000$ &       $20$&   -         & 32.1 & 53.0 & 32.5 & 12.7 & 35.2 & 50.6 \\
    \ding{55}&           $20$&       $20$&   -         & 32.2 & 53.2 & 32.7 & 12.7 & 35.0 & 51.0 \\ 
    \specialrule{0.5pt}{0.7pt}{1.5pt}
    \checkmark&         $20$&       $1000$&      $1000$& 32.2 & 52.9 & 32.9 & 12.8 & 35.1 & 51.1 \\
    \checkmark&       $1000$&         $20$&        $20$& 32.3 & 52.7 & 32.8 & 13.3 & 35.2 & 50.8 \\
    \checkmark&         $20$&         $20$&        $20$& \textbf{33.0} & \textbf{53.6} & \textbf{33.5} & \textbf{13.7} & \textbf{36.3} & \textbf{52.1} \\
    \bottomrule
    \end{tabular}}
  \end{spacing}
  \caption{Ablation Study on the temperature consistency of PE.}
  \label{tab:peca}%
\end{table*}%

==> SAP-DETR Camera Ready/scaling_transformation.tex <==
\begin{table*}[t]
  \centering
    \setlength \tabcolsep{10pt}
    \begin{spacing}{0.7}
    \centering
    \resizebox{0.78\linewidth}{!}{%
    \begin{tabular}{cccccccccc}
    \toprule
    \multirow{2}[2]{*}{\makecell[c]{Concatenate \\ Box Side PE}}&\multicolumn{3}{c}{Scaling Transformation for PE} & \multicolumn{1}{c}{\multirow{2}[2]{*}{AP}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{AP$_{\text{50}}$}}& \multicolumn{1}{c}{\multirow{2}[2]{*}{AP$_{\text{75}}$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{AP$_{\text{S}}$}} & 
    \multicolumn{1}{c}{\multirow{2}[2]{*}{AP$_{\text{M}}$}} &
    \multicolumn{1}{c}{\multirow{2}[2]{*}{AP$_{\text{L}}$}} \\
    \cmidrule{2-4}  
    &\quad\ $\mathbf{T}_k$\ \quad & \quad\ $\mathbf{T}_{qp}$\ \quad & $\mathbf{T}_{qb}$ &       &&&       & & \\
    \toprule
    \ding{55}& \quad\ \tiny{$\Circle$}\ \quad  & \quad\ \tiny{$\Circle$}\ \quad &   -  & 33.3 & 54.4 & 33.9 & 13.1 & 36.3 & 52.2 \\
    \ding{55}& \quad\ \tiny{$\CIRCLE$}\ \quad  & \quad\ \tiny{$\Circle$}\ \quad &   -  & 32.3 & 53.4 & 32.7 & 12.8 & 35.4 & 50.4 \\
    \ding{55}& \quad\ \tiny{$\Circle$}\ \quad  & \quad\ \tiny{$\CIRCLE$}\ \quad &   -  & 34.4 & 55.3 & 35.6 & 14.5 & 37.7 & 53.3 \\
    \ding{55}& \quad\ \tiny{$\CIRCLE$}\ \quad  & \quad\ \tiny{$\CIRCLE$}\ \quad &   -  & 32.6 & 53.7 & 33.1 & 12.2 & 35.5 & 51.1 \\
    \specialrule{0.5pt}{0.7pt}{1.5pt}
    \checkmark& \quad\ \tiny{$\Circle$}\ \quad & \quad\ \tiny{$\Circle$}\ \quad & \tiny{$\Circle$} & 34.0 & 54.5 & 35.0 & 13.9 & 37.1 & 52.8 \\
    \checkmark& \quad\ \tiny{$\CIRCLE$}\ \quad & \quad\ \tiny{$\Circle$}\ \quad & \tiny{$\Circle$} & 33.2 & 54.0 & 34.0 & 13.3 & 36.4 & 51.7 \\
    \checkmark& \quad\ \tiny{$\Circle$}\ \quad & \quad\ \tiny{$\CIRCLE$}\ \quad & \tiny{$\Circle$} & 34.7 & 55.3 & 35.8 & 14.4 & 37.8 & 53.1 \\
    \checkmark& \quad\ \tiny{$\Circle$}\ \quad & \quad\ \tiny{$\Circle$}\ \quad & \tiny{$\CIRCLE$} & 35.1 & 55.1 & 36.7 & 14.9 & 38.2 & 53.5 \\
    \checkmark& \quad\ \tiny{$\CIRCLE$}\ \quad & \quad\ \tiny{$\CIRCLE$}\ \quad & \tiny{$\CIRCLE$} & 32.6 & 53.4 & 33.2 & 12.3 & 35.6 & 52.0 \\
    \checkmark& \quad\ \tiny{$\Circle$}\ \quad & \quad\ \tiny{$\LEFTcircle$}\ \quad & \tiny{$\RIGHTcircle$} & 35.2 & 55.1 & 36.6 & 15.7 & 38.5 & \textbf{53.9 }\\
    \checkmark& \quad\ \tiny{$\Circle$}\ \quad & \quad\ \tiny{$\CIRCLE$}\ \quad & \tiny{$\CIRCLE$} & \textbf{35.2} & \textbf{55.4} & \textbf{36.8} & \textbf{15.8} & \textbf{38.5} & 53.6 \\
    \bottomrule
    \specialrule{0pt}{0pt}{1.5pt}
    \multicolumn{10}{l}{\tiny{$^{\LEFTcircle}$}\!\!\: \normalsize{and} \tiny{$^{\RIGHTcircle}$} \normalsize{denote different independent scaling transformations.}} \\
    \multicolumn{10}{l}{\tiny{$^{\Circle}$} \normalsize{and} \tiny{$^{\CIRCLE}$} \normalsize{denote no scaling and shared scaling transformations, respectively.}} \\
    \bottomrule
    \end{tabular}}
    \end{spacing}
    \caption{Ablation study on the scaling transformation of PE.}
    \vspace{0.25cm}
    \label{tab:scalingtranfer}%
\end{table*}

==> SAP-DETR Camera Ready/tabel1.tex <==



\begin{table*}[htbp]
  \centering
  \setlength \tabcolsep{8pt}
    \begin{spacing}{0.9}
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{lcccccccccc}
    \toprule
    \multicolumn{1}{l}{\textbf{Method}}  & \textbf{Epochs} & \textbf{GFLOPs} & \textbf{\#Params (M)}  & \textbf{MS} & \textbf{AP}&$\textbf{AP}_{50}$&$\textbf{AP}_{75}$ & $\textbf{Ap}_S$&$\textbf{Ap}_M$&$\textbf{Ap}_{L}$ \\
    \specialrule{0.9pt}{1.6pt}{3.6pt}
    \multicolumn{8}{l}{\textit{CNN Backbone with Other Representations}} \\
    \specialrule{0.5pt}{0.8pt}{1.7pt}
    FCOS    & 36    & 177   & -     &    $\checkmark$   & 41.0 &59.8&44.1  & 26.2&44.6&52.2 \\
    Faster R-CNN    & 37    & 180   & 42    &   $\checkmark$    & 40.2&61.0&43.8  & 24.2&43.5&52.0 \\
    Faster R-CNN+    & 109   & 180   & 42     &   $\checkmark$    & 42.0 &62.1&45.5  & 26.6&45.4&53.4 \\
    Mask R-CNN    & 36    & 260   & 44      & $\checkmark$    & 41.0&61.7&44.9  &  \  - \   & \  - \   & \  - \  \\
    Cas. Mask R-CNN          & 36    & 739   & 82    & $\checkmark$    & 46.3&64.3&50.5  & \  - \   & \  - \   & \  - \ \\
    \specialrule{0.5pt}{0.8pt}{1.7pt}
    \multicolumn{8}{l}{\textit{Transformer Model as Neck}} \\
    \specialrule{0.5pt}{0.8pt}{1.7pt}
    DETR-R50   & 50   & 86    & 41     &   \ding{55}   & 34.9 & 55.5 & 36.0  & 14.4 & 37.2 & 54.5 \\
    Deformable DETR-R50  & 50    & 78    & 34    &  \ding{55}     & 39.7&60.1&42.4  & 21.2&44.3&56.0 \\
    Conditional DETR-R50  & 50   & 90    & 44    &     \ding{55}  & 40.9 & 61.8 &43.3  & 20.8&44.6&59.2 \\
    SMCA-DETR-50   & 50    & 86   & 40      &   \ding{55}   & 41.0& \,\  - \,\ & \,\  - \,\     & 21.9&44.3&59.1 \\
    SAM-DETR-w/SMCA-R50 & 50 & 100 & 58 & \ding{55}   & 41.8& 63.2 & 43.9  & 22.1&45.9&60.9 \\
    Anchor-DETR-R50    & 50    & 92.7 & 39     &   \ding{55}    & 42.1&63.1&44.9  & 22.3&46.2&60.0 \\
    DAB-DETR-R50  & 50    & 100   & 44    &   \ding{55}    & 42.6&63.2&45.6  & 21.8&46.2&61.1 \\
    \specialrule{0.5pt}{0.8pt}{1.7pt}
    \multicolumn{8}{l}{\textit{Transformer Model as Neck}} \\
    \specialrule{0.5pt}{0.8pt}{1.7pt}
    DETR-R50   & 50   & 86    & 41     &   \ding{55}   & 34.9 & 55.5 & 36.0  & 14.4 & 37.2 & 54.5 \\
    Deformable DETR-R50  & 50    & 78    & 34    &  \ding{55}     & 39.7&60.1&42.4  & 21.2&44.3&56.0 \\
    Conditional DETR-R50  & 50   & 90    & 44    &     \ding{55}  & 40.9 & 61.8 &43.3  & 20.8&44.6&59.2 \\
    SMCA-DETR-50   & 50    & 86   & 40      &   \ding{55}   & 41.0& \,\  - \,\ & \,\  - \,\     & 21.9&44.3&59.1 \\
    SAM-DETR-w/SMCA-R50 & 50 & 100 & 58 & \ding{55}   & 41.8& 63.2 & 43.9  & 22.1&45.9&60.9 \\
    Anchor-DETR-R50    & 50    & 92.7 & 39     &   \ding{55}    & 42.1&63.1&44.9  & 22.3&46.2&60.0 \\
    DAB-DETR-R50  & 50    & 100   & 44    &   \ding{55}    & 42.6&63.2&45.6  & 21.8&46.2&61.1 \\
    
    % SAP-DETR-R50 & 50 &  & -     &       &   \ding{55} & 
    \bottomrule
    \end{tabular}}
  \end{spacing}
  \caption{Comparison between Transformer necks and representative CNNs with ResNet-50 backbone on COCO 2017 val set. ``GPUs Time'' denotes the training time on our 8$\times$V100 GPUs with 32 batch size;  ``MS'' denotes to multi-scale features.}
  \label{tab:31}
\end{table*}%

==> SAP-DETR Camera Ready/tabel2.tex <==
\begin{table*}[ht]
\centering
  \setlength \tabcolsep{3pt}
    \begin{spacing}{0.79}
    \resizebox{0.95\linewidth}{!}{%
    \begin{tabular}{lccccccccc}
    \toprule
    Method & \#Epochs& \#Params(M) & GFLOPs& AP&AP$_{\text{50}}$&AP$_{\text{75}}$ & AP$_{\text{S}}$&AP$_{\text{M}}$&AP$_{\text{L}}$ \\
    \specialrule{0.9pt}{1.6pt}{3.6pt}
    \multicolumn{10}{l}{\textit{\textbf{3-Layer Encoder-Decoder Transformer Neck with ResNet-50 Backbone}}} \\
    \specialrule{0.5pt}{0.8pt}{1.7pt}
    DETR-R50~\cite{detr}            &  36  & 33   & 82     &   15.8    &  28.0     &   15.4  & 5.3 & 16.7 & 24.6  \\
    Deformable DETR-R50~\cite{deformabledetr} & 36 & 30   & 77    &    37.1   &  57.6     & 39.4   & 18.3 & 40.8 & 51.6  \\
    SMCA-DETR-R50~\cite{smca}       & 12 / 36  & -  & -  & 28.8 / 37.7 & 48.1 / 58.7 & 29.9 / 40.1 & 13.8 / 19.4 & 31.3 / 40.5 & 41.3 / 54.8  \\
    Conditional DETR-R50~\cite{conditionaldetr} & 12 / 36  & 40 & 82 & 29.6 / 37.1 & 48.7 / 57.9 & 30.7 / 39.0 & 13.0 / 17.6 & 32.3 / 40.3 & 43.1 / 55.0  \\
    Anchor DETR-R50~\cite{wang2021anchor}     & 12 / 36  & 31 & 79 & 30.8 / 37.6 & 51.1 / 58.7 & 31.8 / 39.7 & 14.3 / 18.8 & 34.1 / 41.5 & 44.3 / 53.5  \\
    DAB-DETR-R50~\cite{liu2022dab}        & 12 / 36  & 34 & 83 & 32.3 / 39.0 & 51.3 / 58.6 & 34.0 / 41.8 & 15.7 / 20.0 & 35.2 / 42.5 & 45.7 / 56.0  \\
    SAM-DETR-w/SMCA-R50~\cite{zhang2022accelerating} & 12 / 36  & 41 & 89 & 35.1 / 40.4   &   54.7 / 60.7    & 36.7 / 42.7 & 16.0 / 20.2 & 38.4 / 44.4 & 52.1 / 58.3     \\
    SAP-DETR-R50 (Ours) & 12 / 36  & 36 & 84 &  \textbf{36.2} / \textbf{41.2}   &   \textbf{56.2} / \textbf{61.6}    &  \textbf{37.9} / \textbf{43.4}  & \textbf{16.4} / \textbf{21.0}&\textbf{39.5} / \textbf{44.5} & \textbf{53.8} / \textbf{60.1}    \\
    \specialrule{0.9pt}{1.6pt}{3.6pt}
    \multicolumn{10}{l}{\textit{\textbf{6-Layer Encoder-Decoder Transformer Neck with ResNet-50 Backbone}}} \\
    \specialrule{0.5pt}{0.8pt}{1.7pt}
    DETR-R50~\cite{detr}              &  36 & 42 & 89    &    14.0   &    24.4   &  14.0  & 4.2 & 13.7 &  22.5   \\
    Deformable DETR-R50~\cite{deformabledetr}   &   36 & 34 & 81    &   38.0    &    58.2   & 40.4 & 18.5 & 41.7 &  54.2     \\
    SMCA-DETR-R50~\cite{smca}         &  12 / 36 &  - &  -  & 32.4 / 40.1 & 52.3 / 61.4 & 34.0 / 42.8 & 15.5 / 20.3 & 34.9 / 43.3 & 47.7 / 57.1  \\
    Conditional DETR-R50~\cite{conditionaldetr}  &  12 / 36 & 44 & 90  & 33.1 / 40.2 & 53.0 / 61.0 & 34.8 / 42.4 & 14.5 / 19.9 & 35.9 / 43.5 & 49.2 / 58.8 \\
    Anchor DETR-R50~\cite{wang2021anchor}       &  12 / 36 & 37 & 85  & 33.7 / 39.7 & 54.5 / 60.5 & 35.1 / 41.9 & 15.6 / 19.9 & 37.3 / 43.5 & 49.8 / 57.3 \\
    DAB-DETR-R50~\cite{liu2022dab}          &  12 / 36 & 44 & 92  & 34.9 / 41.0 & 55.5 / 61.7 & 36.4 / 43.4 & 16.2 / 21.3 & 38.4 / 44.7 & 51.5 / 58.9 \\
    SAM-DETR-w/SMCA-R50~\cite{zhang2022accelerating}   &  12 / 36 & 59 & 105 & 36.2 / 40.9 & 57.2 / 62.2 & 37.4 / 43.1 & 16.1 / 20.1 & 39.8 / 44.7 & 55.3 / 60.7    \\
    SAP-DETR-R50 (Ours)   &  12 / 36 & 47 & 94 & \textbf{37.5} / \textbf{42.2} & \textbf{58.5} / \textbf{62.7} & \textbf{39.2} / \textbf{44.6} & \textbf{17.3} / \textbf{22.6} & \textbf{40.6} / \textbf{45.7} & \textbf{55.4} / \textbf{60.8}  \\
    % \specialrule{0.9pt}{1.6pt}{3.6pt}
    % \multicolumn{10}{l}{\textit{\textbf{6-Layer Encoder-Decoder Transformer Neck with DC5-ResNet-50 Backbone}}} \\
    % \specialrule{0.5pt}{0.8pt}{1.7pt}
    % SMCA-DETR-DC5-R50~\cite{smca}        & 12 / 36 & -  & -   & 32.6 / 41.1 & 52.8 / 61.9 & 34.1 / 43.7 & 13.8 / 20.7 & 35.0 / 44.5 & 48.9 / 58.0   \\
    % Conditional DETR-DC5-R50~\cite{conditionaldetr}& 12 / 36 & 44 & 193  & 36.6 / 43.2 & 56.4 / 63.6 & 38.5 / 46.1 & 18.1 / 23.1 & 39.8 / 46.8 & 52.7 / 60.8  \\
    % Anchor DETR-DC5-R50~\cite{wang2021anchor}      & 12 / 36 & 37 & 162  & 37.2 / 42.5 & 58.0 / 63.1 & 39.3 / 45.4 & 18.9 / 23.5 & 40.8 / 46.3 & 51.6 / 59.2 \\
    % DAB-DETR-DC5-R50~\cite{liu2022dab}         & 12 / 36 & 44 & 197  & 37.4 / 43.9 & 57.5 / 64.2 & 39.8 / 47.0 & 19.7 / 25.2 & 40.6 / 47.5 & 53.3 / 60.2 \\
    % SAM-DETR-w/SMCA-DC5-R50~\cite{zhang2022accelerating}  & 12 / 36 & 59 & 219 & 40.2 / 44.2 & 60.8 / 65.0 & 42.4 / 47.0 & 21.3 / 25.3 & 43.8 / 47.8 & \ \textbf{58.3} / \textbf{62.3 }  \\
    % SAP-DETR-DC5-R50 (Ours)  & 12 / 36 & 48 & 200 & \textbf{41.0} / \textbf{45.4} & \textbf{60.8} / \textbf{65.1} & \textbf{43.5} / \textbf{48.3} & \textbf{23.1} / \textbf{26.2} & \textbf{44.5} / \textbf{49.3} & 57.8 / 61.9 \\
    \bottomrule
    \end{tabular}}
    \end{spacing}
    \caption{Comparison between Transformer necks. Based on ResNet-50 backbone, all models are trained by the official source codes with their original settings and evaluated on COCO \texttt{val2017}. All models uses 400 queries except Anchor DETR, while Anchor DETR uses 200 queries with 2 pattern embeddings. GFLOPs and Params are measured by Detectron2\protect\footnotemark.}
    \label{tab:31}
\end{table*}%
\footnotetext{https:// github.com/facebookresearch/detectron2}

==> SAP-DETR Camera Ready/tabel3.tex <==
\begin{table*}[ht]
\centering
  \setlength \tabcolsep{5pt}
    \begin{spacing}{0.85}
    \resizebox{0.93\linewidth}{!}{%
    \begin{tabular}{lccccccccc}
    \toprule
    Method & \#Epochs& \#Params(M) & GFLOPs& AP&AP_{\text{50}}&AP_{\text{75}} & AP_{\text{S}}&AP_{\text{M}}&AP_{\text{L}} \\
    \specialrule{0.9pt}{1.6pt}{3.6pt}
    \multicolumn{10}{l}{\textit{\textbf{3Encoder-3Decoder Transformer Neck with ResNet-50 Backbone}}} \\
    \specialrule{0.5pt}{0.8pt}{1.7pt}
    DETR-R50 & 12  & 33   & 82    &       &       &    &&&     \\
    Deformable DETR-R50& 12 & 30   & 77    &       &       &  &&&       \\
    SMCA-DETR-R50       & 12  & -  & -  & 28.2 & 47.6 & 29.1 & 13.3 & 31.1 & 39.7  \\
    Conditional DETR-R50& 12  & 40 & 82 & 28.4 & 47.1 & 29.3 & 12.8 & 31.2 & 42.2  \\
    Anchor DETR-R50     & 12  & 31 & 79 & 29.9 & 50.2 & 30.6 & 13.7 & 33.3 & 42.7  \\
    DAB-DETR-R50        & 12  & 34 & 87 & 31.3 & 50.0 & 32.5 & 14.5 & 34.3 & 45.3  \\
    SAM-DETR-w/SMCA-R50 & 12  & 41 & 89 &    34.1   &   53.8    & \textbf{35.9} & \textbf{16.5} & 37.5 & 51.0     \\
    SAP-DETR-R50 (Ours) & 12  & 36 & 88 &  \textbf{34.6}     &   \textbf{54.8}    &  35.8  &15.0&\textbf{38.1}& \textbf{53.0}   \\
    \specialrule{0.5pt}{0.8pt}{1.7pt}
    DETR-R50 & 36  & 33   & 82    &       &       &    &&&     \\
    Deformable DETR-R50& 36 & 30   & 77    &       &       &  &&&       \\
    SMCA-DETR-R50      & 36 &    &       & 36.5 & 57.5 & 38.7 & 18.7 & 39.6 & 52.4   \\
    Conditional DETR-R50& 36  & 40   & 82 & 36.8 & 57.4 & 39.0 & 17.9 & 39.9 & 54.1      \\
    Anchor DETR-R50    & 36 & 31 & 79 & 36.6 & 57.8 & 38.5 & 18.1 & 40.4 & 52.6    \\
    DAB-DETR-R50       & 36 & 34 & 87 & 39.0 & 58.6 & 41.8 & 20.0 & 42.5 & 56.0  \\
    SAM-DETR-w/SMCA-R50& 36 & 41 & 89 & \textbf{40.2} & \textbf{60.5} & \textbf{42.5} & \textbf{20.2} & \textbf{44.3} & 58.3     \\
    SAP-DETR-R50 (Ours)& 36 & 36 & 88 & 39.8 & 60.3 & 41.9 & 18.2 & 43.7 & \textbf{59.2}   \\
    \specialrule{0.9pt}{1.6pt}{3.6pt}
    \multicolumn{10}{l}{\textit{\textbf{6Encoder-6Decoder Transformer Neck with ResNet-50 Backbone}}} \\
    \specialrule{0.5pt}{0.8pt}{1.7pt}
    DETR-R50& 12  & 42   & 89    &       &       &     &&&   \\
    Deformable DETR-R50& 12 & 34   & 81    &       &       &    &&&   \\
    SMCA-DETR-R50         & 12 &  - &  -  & 32.4 & 52.3 & 34.0 & 15.5 & 34.9 & 47.7  \\
    Conditional DETR-R50  & 12 & 44 & 90  & 33.1 & 53.0 & 34.8 & 14.5 & 35.9 & 49.2 \\
    Anchor DETR-R50       & 12 & 41 & 89  & 33.7 & 54.5 & 35.1 & 15.6 & 37.3 & 49.8 \\
    DAB-DETR-R50          & 12 & 44 & 96  & 34.9 & 55.5 & 36.4 & 16.2 & 38.4 & 51.5 \\
    SAM-DETR-w/SMCA-R50   & 12 & 59 & 105 & 36.2 & \textbf{57.2} & 37.4 & 16.1 & 39.8 & 55.3    \\
    SAP-DETR-R50 (Ours)   & 12 & 47 & 104 & \textbf{36.6} & 57.0 & \textbf{38.1} & \textbf{16.6} & \textbf{40.4} & \textbf{55.8}  \\
    \specialrule{0.9pt}{1.6pt}{3.6pt}
    DETR-R50             & 36  & 42   & 89    &       &       &     &&&   \\
    Deformable DETR-R50  & 36 & 34   & 81    &       &       &    &&&   \\
    SMCA-DETR-R50        & 36 & -  & -   & 40.1 & 61.4 & 42.8 & 20.3 & 43.3 & 57.1   \\
    Conditional DETR-R50 & 36 & 44 & 90  & 40.2 & 61.0 & 42.4 & 19.9 & 43.5 & 58.8  \\
    Anchor DETR-R50      & 36 & 41 & 89  & 39.7 & 60.5 & 41.9 & 19.9 & 43.5 & 57.3 \\
    DAB-DETR-R50         & 36 & 44 & 96  &  &  &  &  &  &  \\
    SAM-DETR-w/SMCA-R50  & 36 & 59 & 105 & 40.9 & \textbf{62.2} & 43.1 & 20.1 & 44.7 & \textbf{60.7}   \\
    SAP-DETR-R50 (Ours)  & 36 & 47 & 104 & \textbf{41.1} & 61.4 & 43.1 & \textbf{20.2} & \textbf{45.6} & 60.4  \\
    % \specialrule{0.9pt}{1.6pt}{3.6pt}
    % \multicolumn{10}{l}{\textit{\textbf{6Encoder-6Decoder Transformer Neck with ResNet-50-DC5 Backbone}}} \\
    % \specialrule{0.5pt}{0.8pt}{1.7pt}
    % DETR-R50-DC5& 12  & 42   & 89    &       &       &     &&&   \\
    % Deformable DETR-R50-DC5& 12 & 34   & 81    &       &       &    &&&   \\
    % Conditional DETR-R50-DC5 &12 & 44   & 90    &       &       &   &&&   \\
    % SMCA-DETR-R50-DC5& 12 &       &       &       &       &    &&&   \\
    % SAM-DETR-w/SMCA-R50-DC5& 12& 59   & 105   &       &       &   &&&    \\
    % Anchor DETR-R50-DC5& 12 & 41   & 89    &       &       &    &&&   \\
    % DAB-DETR-R50-DC5& 12  & 44  & 96    &       &       &     &&&  \\
    % SAP-DETR-R50-DC5 (Ours)& 12 & 47   & 104   &       &       &    &&&   \\
    \specialrule{0.5pt}{0.8pt}{1.7pt}
    \end{tabular}
    }
  \end{spacing}
  \caption{Comparison between Transformer necks and representative CNNs with ResNet-50 backbone on COCO 2017 val set.}
  \label{tab:31}
\end{table*}%


==> SAP-DETR Camera Ready/tabel4.tex <==
\begin{table*}[t]
  \centering
  \setlength \tabcolsep{9pt}
  \begin{spacing}{0.7}
  \resizebox{0.95\linewidth}{!}{%
    \begin{tabular}{lcccccccccc}
    \toprule
    \multicolumn{1}{l}{Comment} &Movable & Inner Loss & PECA & SDG %& \multicolumn{1}{l}{\makecell[l]{First indep. Head$_{\text{cls}}$  \\ \ \& Indep. Head$_{\text{box}}$}} 
    & \multicolumn{1}{c}{AP} & \multicolumn{1}{c}{AP$_{\text{50}}$} & \multicolumn{1}{c}{AP$_{\text{75}}$} & \multicolumn{1}{c}{AP$_{\text{S}}$} & \multicolumn{1}{c}{AP$_{\text{M}}$} & \multicolumn{1}{c}{AP$_{\text{L}}$} \\
    \toprule
    SAP-DETR (\textbf{Ours})          & \checkmark & \checkmark & \checkmark & \checkmark  & \textbf{36.2} & 56.2     & \textbf{37.9} &   \textbf{16.4}    &   \textbf{39.5}    & \textbf{53.8} \\
    % \quad $-$Indep. Head & \checkmark & \checkmark & \checkmark & \checkmark     &            & 35.6  & 56.0  & 37.2  & 16.3  & 38.2  & 52.3 \\
    \quad $-$SDG             & \checkmark & \checkmark & \checkmark &             & 35.6  & 56.2  & 36.9  & 16.3  & 38.9  & 52.7 \\
    \quad $-$PECA            & \checkmark & \checkmark &            & \checkmark  & 34.8  & 55.5  & 36.0  & 15.7  & 37.3  & 52.0 \\
    \quad $-$PECA \& SDG     & \checkmark & \checkmark &            &             & 34.0  & 54.9  & 35.3  & 15.0  & 36.7  & 51.5 \\
    \quad $-$Movable       &            & \checkmark & \checkmark & \checkmark   & 35.2  & 55.4  & 36.8  & 15.8  & 38.5  & \textbf{53.8} \\
    \quad $-$Inner Loss      & \checkmark &            & \checkmark & \checkmark & 35.9  & \textbf{56.3}  & 37.4  & 16.2  & 39.3  & 52.5 \\
    \specialrule{0.5pt}{1.5pt}{2pt}
    DAB-DETR (Baseline)& \textbf{-} & \textbf{-} & \textbf{-} & \textbf{-}  & 32.3  & 51.3  & 34.0  & 15.7  & 35.2  & 45.7 \\
    \quad $+$Salient Point Concept & \textbf{-} & \textbf{-} & \textbf{-} & \textbf{-}  & 33.5  & 54.3  & 35.1  & 14.3  & 36.5  & 51.0 \\
    \bottomrule
    \end{tabular}}
    \end{spacing}
    \caption{Ablation on each components}
    \label{tab:effectiveness}%
\end{table*}%


==> SAP-DETR Camera Ready/tabel5.tex <==
\begin{table}[t]
  \centering
  \setlength \tabcolsep{2pt}
  \begin{spacing}{0.8}
    \centering
    \resizebox{1\linewidth}{!}{%
    \begin{tabular}{cccccc}
    \toprule
    Inner Cost ($\mathcal{L}_{\text{inner}}$)& Movable within Grid ($\boldsymbol{s}_{\text{grid}}$) & AP    & AP$_\text{S}$    & AP$_\text{M}$    & AP$_\text{L}$ \\
    \toprule
               &            &    35.9        & \textbf{17.0} &     38.8      &  52.7 \\
    \checkmark &            &    26.3        &   11.3        &     28.0      &  39.5 \\
    \checkmark & \checkmark &  \textbf{36.2} & 16.4          & \textbf{39.5} &  \textbf{53.8} \\
    \bottomrule
    \end{tabular}}
    \vspace{-0.1cm}
    \caption{Ablation on scaling factor of grid}
    \vspace{0.15cm}
    \label{tab:ablation_sfg}
    \end{spacing}
\end{table}%



\begin{table}[t]
  \centering
  \setlength \tabcolsep{7pt}
  \begin{spacing}{0.8}
    \centering
    \resizebox{1\linewidth}{!}{%
    \begin{tabular}{cccccc}
    \toprule
    \ \ PECA\  \   & Scaling Factor of SDG & AP    & AP$_\text{S}$    & AP$_\text{M}$    & AP$_\text{L}$ \\
    \toprule
               &            &  33.6          &  14.7         &     36.0      &  50.7 \\
    \checkmark &            &  35.7          &  \textbf{17.5}         &     38.8      &  52.6 \\
    \checkmark & \checkmark &  \textbf{36.2} & 16.4 & \textbf{39.5} &  \textbf{53.8} \\
    \bottomrule
    \end{tabular}}
    \caption{Ablation on scaling factor of SDG}
    \vspace{-0.1cm}
    \label{tab:ablation_sdg}
    \end{spacing}
\end{table}%

==> SAP-DETR Camera Ready/tabel6.tex <==
\begin{table*}[t]
\centering
  \setlength \tabcolsep{6pt}
    \begin{spacing}{0.7}
    \resizebox{0.95\linewidth}{!}{%
    \begin{tabular}{lcccccccccc}
    \toprule
    Method & \#Epochs& \#Params(M) & GFLOPs& AP&AP$_{\text{50}}$&AP$_{\text{75}}$ & AP$_{\text{S}}$&AP$_{\text{M}}$&AP$_{\text{L}}$&Infer. Time(s/img)$^\dag$\\%&\makecell[c]{Training Time \\ (GPU hour/Epoch)} \\
    \specialrule{0.9pt}{1.6pt}{3.6pt}
    \multicolumn{11}{l}{\textit{\textbf{ResNet-50 Backbone}}} \\
    \specialrule{0.5pt}{0.8pt}{1.7pt}
    Faster RCNN-FPN-R50~\cite{fastercnn,fpn}   & 108& 42 & 180 & 42.0 & 62.1 & 45.5 & 26.6 & 45.5 & 53.4&0.039 \\
    DETR-R50~\cite{detr}              & 500& 41 & 86  & 42.0 & 62.4 & 44.2 & 20.5 & 45.8 & 61.1&0.040 \\
    Deformable DETR-R50~\cite{deformabledetr}   & 50 & 34 & 78  & 39.4 & 59.6 & 42.3 & 20.6 & 43.0 & 55.5&0.043 \\
    SMCA-DETR-R50~\cite{smca}         & 50 & 42 & 86  & 41.0 & -    & -    & 21.9 & 44.3 & 59.1& 0.045\\
    Conditional DETR-R50~\cite{conditionaldetr}  & 50 & 44 & 90  & 40.9 & 61.8 & 43.3 & 20.8 & 44.6 & 59.2&0.057 \\
    Anchor DETR-R50~\cite{wang2021anchor}       & 50 & 39 & 85  & 42.1 & 63.1 & 44.9 & 22.3 & 46.2 & 60.0&0.050 \\
    DAB-DETR-R50~\cite{liu2022dab}          & 50 & 44 & \ \,\:90$^\dag$  & 42.2 & 63.1 & 44.7 & 21.5 & 45.7 & 60.3&0.059 \\
    SAM-DETR-w/SMCA-R50~\cite{zhang2022accelerating}   & 50 & 58 & 100 & 41.8 & 63.2 & 43.9 & 22.1 & 45.9 & 60.9&0.065 \\
    SAP-DETR-R50 (\textbf{Ours})   & 50 & 47 & 92  & \textbf{43.1} & \textbf{63.8} & \textbf{45.4} & \textbf{22.9} & \textbf{47.1} & \textbf{62.1}&0.063 \\
    \specialrule{0.9pt}{1.6pt}{3.6pt}
    \multicolumn{11}{l}{\textit{\textbf{ResNet-101 Backbone}}} \\
    \specialrule{0.5pt}{0.8pt}{1.7pt}
    Faster RCNN-FPN-R101~\cite{fastercnn,fpn}  & 108& 60 & 246  & 44.0 & 63.9 & 47.8 & 27.2 & 48.1 & 56.0&0.050 \\
    DETR-R101~\cite{detr}             & 500& 60 & 152  & 43.5 & 63.8 & 46.4 & 21.9 & 48.0 & 61.8&0.066 \\
    Conditional DETR-R101~\cite{conditionaldetr} & 50 & 63 & 156  & 42.8 & 63.7 & 46.0 & 21.7 & 46.6 & 60.9&0.070 \\
    Anchor DETR-R101~\cite{wang2021anchor}       & 50 & 58 & 150   & 43.5 & 64.3 & 46.6 & 23.2 & 47.7 & 61.4&0.068 \\
    DAB-DETR-R101~\cite{liu2022dab}         & 50 & 63 & \,\:157$^\dag$  & 43.5 & 63.9 & 46.6 & 23.6 & 47.3 & 61.5&0.072 \\
    SAP-DETR-R101 (\textbf{Ours})  & 50 & 67 & 158 & \textbf{44.4} & \textbf{64.9} & \textbf{47.1} & \textbf{24.1} & \textbf{48.7} & \textbf{63.1}&0.078 \\
    \specialrule{0.9pt}{1.6pt}{3.6pt}
    \multicolumn{11}{l}{\textit{\textbf{DC5-ResNet-50 Backbone}}} \\
    \specialrule{0.5pt}{0.8pt}{1.7pt}
    DETR-DC5-R50~\cite{detr}             & 500& 41 & 187  & 43.3 & 63.1 & 45.9 & 22.5 & 47.3 & 61.1&0.087 \\
    Conditional DETR-DC5-R50~\cite{conditionaldetr} & 50 & 44 & 195  & 43.8 & 64.4 & 46.7 & 24.0 & 47.6 & 60.7&0.093 \\
    Anchor DETR-DC5-R50~\cite{wang2021anchor}      & 50 & 39 & 151  & 44.2 & 64.7 & 47.5 & 24.7 & 48.2 & 60.6&0.069 \\
    DAB-DETR-DC5-R50~\cite{liu2022dab}         & 50 & 44 & \,\:194$^\dag$  & 44.5 & 65.1 & 47.7 & 25.3 & 48.2 & 62.3&0.094 \\
    SAM-DETR-w/SMCA-DC5-R50~\cite{zhang2022accelerating}  & 50 & 58 & 210 & 45.0 & 65.4 & 47.9 & 26.2 & 49.0 & \textbf{63.3}&0.126   \\
    SAP-DETR-DC5-R50 (\textbf{Ours})  & 50 & 47 & 197 & \textbf{46.0} & \textbf{65.5} & \textbf{48.9} & \textbf{26.4} & \textbf{50.2} & 62.6&0.116 \\
    \specialrule{0.9pt}{1.6pt}{3.6pt}
    \multicolumn{11}{l}{\textit{\textbf{DC5-ResNet-101 Backbone}}} \\
    \specialrule{0.5pt}{0.8pt}{1.7pt}
    DETR-DC5-R101~\cite{detr}             & 500& 60 & 253  & 44.9 & 64.7 & 47.7 & 23.7 & 49.5 & 62.3&0.101 \\
    Conditional DETR-DC5-R101~\cite{conditionaldetr} & 50 & 63 & 262  & 45.0 & 65.6 & 48.4 & 26.1 & 48.9 & 62.8&0.105 \\
    Anchor DETR-DC5-R101~\cite{wang2021anchor}      & 50 & 58 & 227    & 45.1 & 65.7 & 48.8 & 25.8 & 49.4 & 61.6&0.083 \\
    DAB-DETR-DC5-R101~\cite{liu2022dab}         & 50 & 63 & \,\:263$^\dag$  & 45.8 & 65.9 & 49.3 & 27.0 & 49.8 & 63.8&0.110 \\
    SAP-DETR-DC5-R101 (\textbf{Ours})  & 50 & 67 & 266 & \textbf{46.9} & \textbf{66.7} & \textbf{50.5} & \textbf{27.9} & \textbf{51.3} & \textbf{64.3}&0.130 \\
    \bottomrule
    \end{tabular}}
    \end{spacing}
    \caption{Comparison of Transformer necks with 300 queries on COCO \texttt{val2017}. All results are reported from their original paper. All models uses 300 queries except Anchor DETR, while Anchor DETR uses 100 queries with 3 pattern embeddings. All inference speeds are measured by a single Nvidia A100 GPU. $^\dag$ denotes the results are measured by ourselves.}
        \vspace{-0.15cm}
    \label{tab:50epoch}
\end{table*}%

==> SAP-DETR Camera Ready/table_mask.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet4'
\begin{table}[t]
 \vspace{0.3cm}
  \centering
  \setlength \tabcolsep{3pt}
    \begin{spacing}{1}
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{c|c|c|c|c|c|c}
    \shline
    \hline
    Mode&No Mask & Layer 0 & Layer 1 & Layer 2 & Layer 3 & Layer 4 \\
    \hline
    AP&   0   &   -0.9    &    -0.2   &   -0.1    &   +0.1    & 0 \\
    \hline
    % GFLOPs&8.54/94      &  8.07/93.6     &   8.17/93.7    &  8.26/93.8     &  8.35/93.9    & 8.45/94 \\
    GFLOPs&8.54      &  8.07     &   8.17    &  8.26     &  8.35    & 8.45 \\
    \shline
    \hline
    Mode&Layer 1,2 & Layer 1,3 & Layer 1,4 & Layer 2,3 & Layer 2,4 & Layer 3,4 \\
    \hline
    AP&    -0.6  &   \textbf{+0.2}    &   -0.4    &   +0    &   -0.4    &  +0.1\\
    \hline
    % GFLOPs&  8.03/93.6    & 8.07/93.7      &  8.12/93.7     &   8.17/93.8    &   8.21/93.8    & 8.31/93.9 \\
    GFLOPs&  8.03   & 8.07      &  8.12     &   8.17    &   8.21    & 8.31 \\
    \shline
    \hline
    \end{tabular}}
  \end{spacing}
  \caption{Ablation of mask layer. The GFLOPs of the decoder layer and the change AP relative to no mask.}
  \label{tab:mask}%
\end{table}%


==> SAP-DETR Camera Ready/table_movepoint.tex <==
% \begin{table}[t]
%   \centering
%   \setlength \tabcolsep{2pt}
%     \begin{spacing}{0.8}
%     \resizebox{0.95\linewidth}{!}{%
%     \begin{tabular}{c|lcccc}
%     \toprule
%     \specialrule{0pt}{0.9pt}{3pt}
%     Structure & \multicolumn{1}{l}{Comments} & AP & AP$_{\text{S}}$ & AP$_{\text{M}}$ &  AP$_{\text{L}}$\\
%     \specialrule{0pt}{0.9pt}{1.3pt}
%     \toprule
%     \multirow{3}[1]{*}{\makecell[c]{3-3 Layer \\ SAP-DETR}} & Fixed Point & 40.1 & 19.2 & 44.1 & 59.0 \\
%     % fake
%     & Offset within image & 39.8 (\textcolor{csam}{-0.3}) & 19.6 (\textcolor{red}{+0.4}) & 44.0 (\textcolor{csam}{-0.1}) & 58.0 (\textcolor{csam}{-1.0})\\
%     & Offset within grid  & \textbf{40.8} (\textcolor{red}{\textbf{+0.7}}) & \textbf{20.9} (\textcolor{red}{\textbf{+1.7}}) & \textbf{44.3} (\textcolor{red}{\textbf{+0.2}}) & \textbf{59.0} \\
%     \specialrule{1pt}{0.9pt}{1.3pt}
%     \multirow{3}[1]{*}{\makecell[c]{6-6 Layer \\ SAP-DETR}} & Fixed Point         & 41.3 & 20.0 & \textbf{45.8} & \textbf{61.5} \\
%     % fake
%     & Offset within image & 41.1 (\textcolor{csam}{-0.2}) & 20.3 (\textcolor{red}{+0.3}) & 45.2 (\textcolor{csam}{-0.6}) & 60.3 (\textcolor{csam}{-1.2})\\
%     & Offset within grid  & \textbf{42.0} (\textcolor{red}{\textbf{+0.7}}) & \textbf{21.9} (\textcolor{red}{\textbf{+1.9}}) & 45.5 (\textcolor{csam}{-0.3}) & 60.8 (\textcolor{csam}{-0.7}) \\
%      \specialrule{0pt}{2pt}{1pt}
%      \bottomrule
%     \end{tabular}}
%   \end{spacing}
%   \caption{Ablation on reference point offsets.}
%   \label{tab:effectiveness}
% \end{table}%



\begin{table}[t]
  \centering
  \setlength \tabcolsep{6pt}
    \begin{spacing}{1}
    \resizebox{0.95\linewidth}{!}{%
    \begin{tabular}{c|lcccc}
    \toprule
    \specialrule{0pt}{0.9pt}{3pt}
    Structure & \multicolumn{1}{l}{Comments} & AP & AP$_{\text{S}}$ & AP$_{\text{M}}$ &  AP$_{\text{L}}$\\
    \specialrule{0pt}{0.9pt}{1.3pt}
    \toprule
    \multirow{3}[1]{*}{\makecell[c]{3-3 Layer \\ SAP-DETR}} & \makecell[l]{Indep. box head \\ \& Shared cls. head} & 40.1 & 19.2 & 44.1 & 59.0 \\
    \specialrule{0pt}{0.5pt}{1pt}
    & \makecell[l]{Indep. box head \\ \& First Indep. cls. head} & \textbf{40.4} & \textbf{19.2} & \textbf{44.6} & \textbf{59.6} \\
    
    \specialrule{0.5pt}{0.8pt}{1.2pt}
    
    \multirow{3}[1]{*}{\makecell[c]{6-6 Layer \\ SAP-DETR}} & \makecell[l]{Indep. box head \\ \& Shared cls. head} & 41.2 & \textbf{20.0} & 45.6 & 61.2 \\
    \specialrule{0pt}{0.5pt}{1pt}
    & \makecell[l]{Indep. box head \\ \& First Indep. cls. head} & \textbf{41.3} & 19.9 & \textbf{45.8} & \textbf{61.1} \\
     \specialrule{0pt}{1.5pt}{0.8pt}
     \bottomrule
    \end{tabular}}
  \end{spacing}
  \caption{Ablation on classification head.}
  \label{tab:effectiveness}
\end{table}%



==> SAP-DETR Camera Ready/table_sap-dn-detr.tex <==
% \begin{table*}[ht]
% \centering
%   \setlength \tabcolsep{5pt}
%     % \begin{spacing}{0.95}
%     \resizebox{0.97\linewidth}{!}{%
%     \begin{tabular}{lccccccccc}
%     \toprule
%     Method & \#Epochs& \#Params(M) & GFLOPs& AP&AP$_{\text{50}}$&AP$_{\text{75}}$ & AP$_{\text{S}}$&AP$_{\text{M}}$&AP$_{\text{L}}$ \\
%     \specialrule{0.9pt}{1.6pt}{3.6pt}
%     \multicolumn{10}{l}{\textit{\textbf{ResNet Backbone}}} \\
%     \specialrule{0.5pt}{0.8pt}{1.7pt}
%     DN-DETR-R50~\cite{li2022dn}          & 12   & 44   & 90    & 38.3   & 58.6    & 40.5   & 18.4  & 41.6 & 57.1  \\
%     \rowcolor{gray!25} SAP-DN-DETR-R50      & 12   & 47   & 92    & 39.3 (+1.0)   & 59.5 (+0.9)     & 41.4 (+0.9)   & 18.0 (-0.4) & 42.6 (+1.0) & 58.4 (+1.3)  \\
%     DN-DETR-R101~\cite{li2022dn}        & 12   & 63   & 157    & 40.5   & 60.8     & 43.0   & 19.3 & 44.3 & 59.6  \\
%     \rowcolor{gray!25} SAP-DN-DETR-R101     & 12   & 67   & 158    & 40.7 (+0.2)  & 60.9 (+0.1)    & 43.0 (+0.0)  & 19.3 (+0.0) & 45.2 (+0.9) & 59.7 (+0.1) \\
%     \specialrule{0.9pt}{1.6pt}{3.6pt}
%     \multicolumn{10}{l}{\textit{\textbf{DC5-ResNet Backbone}}} \\
%     \specialrule{0.5pt}{0.8pt}{1.7pt}
%     DN-DETR-DC5-R50~\cite{li2022dn}      & 12   & 44    & 194     & 41.7   & 61.4     & 44.1   & 21.2 & 45.0 & 60.2  \\
%     \rowcolor{gray!25} SAP-DN-DETR-DC5-R50  & 12   & 47   & 197    & 43.3 (+1.6)  & 62.5 (+1.1)    & 46.2 (+2.1)  & 23.8 (+2.6) & 46.6 (+1.6) & 61.2 (+1.0) \\
%     DN-DETR-DC5-R101~\cite{li2022dn}     & 12   & 63   & 263    & 43.4   & 61.9     & 47.2   & 24.8  & 46.8 & 59.4  \\
%     \rowcolor{gray!25} SAP-DN-DETR-DC5-R101 & 12   & 67   & 266    & 43.9 (+0.5)  & 62.9 (+1.0)    & 46.9 (-0.3)  & 24.5 (-0.3) & 48.1 (+1.3) & 61.4 (+2.0)  \\
%     \bottomrule
%     \end{tabular}}
%     % \end{spacing}
%     \caption{Comparison with DN-DETR on COCO \texttt{val2017}. Based on ResNet backbone, the models are trained by the official source codes with their original settings. The results of ResNet-DC backbone are reported from the original paper. The denoising training is a test free strategy, and all models uses 300 queries whose Params and GFLOPs are consistent with both DAB-DETR and SAP-DETR.}
%     \label{tab:sap-dn-detr}
% \end{table*}%


\begin{table*}[ht]
\centering
  \setlength \tabcolsep{4.6pt}
    \begin{spacing}{0.9}
    \resizebox{0.95\linewidth}{!}{%
    \begin{tabular}{ccccccccccc}
    \toprule
    \multirow{2}[1]{*}{Backbone} & \multirow{2}[1]{*}{Epoch} & \multirow{2}[1]{*}{w/ SAP} & \multicolumn{2}{c}{DN-DETR~\cite{li2022dn}} &\quad& \multicolumn{2}{c}{DINO (Single-Scale)~\cite{zhang2022dino}} &\quad& \multicolumn{2}{c}{Group DETR~\cite{chen2022group}} \\
    \specialrule{0pt}{2pt}{0pt}
    \cline{4-5} \cline{7-8} \cline{10-11}
    \specialrule{0pt}{0pt}{2pt}
    &&&  AP\ /\ AP$_{\text{50}}$\ /\ AP$_{\text{75}}$ & AP$_{\text{S}}$\ /\ AP$_{\text{M}}$\ /\ AP$_{\text{L}}$ &\quad&
    AP\ /\ AP$_{\text{50}}$\ /\ AP$_{\text{75}}$ & AP$_{\text{S}}$\ /\ AP$_{\text{M}}$\ /\ AP$_{\text{L}}$  &\quad&
    AP\ /\ AP$_{\text{50}}$\ /\ AP$_{\text{75}}$ & AP$_{\text{S}}$\ /\ AP$_{\text{M}}$\ /\ AP$_{\text{L}}$ \\
    \specialrule{0.9pt}{1.6pt}{3.6pt}
    % \multicolumn{5}{l}{\textit{\textbf{ResNet Backbone}}} \\
    
    \multirow{2}[0]{*}{R50}    &\multirow{2}[0]{*}{12}&& 38.3  / 58.6   / 40.5   & 18.4  / 41.6 / 57.1 
    &\quad& 39.7  / 58.3   / 42.4   & 19.1  / 43.7 / 57.1 
    &\quad& 39.1  / \;\, - \;\, / \;\, - \;\,  & 19.7  / 42.5 / 56.8  \\
    
    &&\checkmark (\textbf{Ours})& \cellcolor{gray!25}\textbf{39.5}  / \textbf{59.7}   / \textbf{41.5}   &\cellcolor{gray!25} \textbf{18.7}  / \textbf{42.8} / \textbf{59.0} 
    &\cellcolor{gray!25}\quad &\cellcolor{gray!25}\textbf{40.0}  / \textbf{60.1}   / 42.1   &\cellcolor{gray!25} \textbf{20.2}  / 43.4 / \textbf{58.5} 
    &\cellcolor{gray!25}\quad &\cellcolor{gray!25}\textbf{39.8}  / \textbf{60.2}  / \textbf{42.0}   &\cellcolor{gray!25} \textbf{20.2}  / \textbf{43.5} / \textbf{58.6}  \\

    \specialrule{0.5pt}{0.8pt}{1.7pt}
    \multirow{2}[0]{*}{R101}   &\multirow{2}[0]{*}{12}&& 40.5  / 60.8   / 43.0   & 19.3  / 44.3 / 59.6 
    &\quad& 41.9  / 60.8   / 44.4   & 22.5  / 46.3 / 59.5 
    &\quad& \;\, - \;\,  / \;\, - \;\,   / \;\, - \;\,   & \;\, - \;\,  / \;\, - \;\, / \;\, - \;\, \\
    
    &&\checkmark(\textbf{Ours})& \cellcolor{gray!25}\textbf{41.0}  / \textbf{61.2}   / \textbf{43.4}   &\cellcolor{gray!25} \textbf{19.8}  / \textbf{45.3} / \textbf{60.0} 
    &\cellcolor{gray!25}\quad &\cellcolor{gray!25}41.5  / \textbf{61.4}   / 43.6   &\cellcolor{gray!25} 20.3 / 45.2 / \textbf{60.0}
    &\cellcolor{gray!25}\quad &\cellcolor{gray!25}\textbf{41.1}  / \textbf{61.5}   /\textbf{ 43.4}   &\cellcolor{gray!25} \textbf{20.5} / \textbf{45.5} / \textbf{59.4} \\
    
    \specialrule{0.5pt}{0.8pt}{1.7pt}
    \multirow{2}[0]{*}{R50-DC} &\multirow{2}[0]{*}{12}&& 41.7  / 61.4  / 44.1   & 21.2  / 45.0 / 60.2 
    &\quad& 43.6  / 61.4  / 47.0   & 24.8  / 47.3 / 59.5
    &\quad& 41.9  / \;\, - \;\, / \;\, - \;\,  & 23.3  / 45.6 / 58.4  \\
    
    &&\checkmark(\textbf{Ours})&  \cellcolor{gray!25}\textbf{43.6}  / \textbf{62.5}  / \textbf{46.2}   &\cellcolor{gray!25} \textbf{23.3}  / \textbf{47.3} / \textbf{61.0} 
    &\cellcolor{gray!25}\quad  &\cellcolor{gray!25}\textbf{44.0}  / \textbf{63.1}  / 46.5   &\cellcolor{gray!25} \textbf{24.8} / \textbf{47.3} / \textbf{61.1}
    &\cellcolor{gray!25}\quad  &\cellcolor{gray!25}\textbf{43.9}  / \textbf{63.2}  / \textbf{46.8}   &\cellcolor{gray!25} \textbf{24.5}  / \textbf{47.6} / \textbf{61.3}  \\
    
    \specialrule{0.5pt}{0.8pt}{1.7pt}
    \multirow{2}[0]{*}{R101-DC}&\multirow{2}[0]{*}{12}&& 43.4  / 61.9  / 47.2   & 24.8  / 46.8 / 59.4 
    &\quad&  45.4  / 63.5  / 49.2   & 26.4  / 49.5 / 61.1
    &\quad&  \;\, - \;\,  /\;\, - \;\,  / \;\, - \;\,   & \;\, - \;\,  / \;\, - \;\, / \;\, - \;\, \\
    
    &&\checkmark(\textbf{Ours})&\cellcolor{gray!25} \textbf{44.6}  / \textbf{63.9}  / \textbf{48.0}   &\cellcolor{gray!25} \textbf{25.5}  / \textbf{48.9} / \textbf{62.5} 
    &\cellcolor{gray!25}\quad  &\cellcolor{gray!25}\textbf{45.6}  / \textbf{64.5}  / 48.7   &\cellcolor{gray!25} 25.0  / \textbf{49.7} / \textbf{62.5}
    &\cellcolor{gray!25}\quad  &\cellcolor{gray!25}\textbf{44.4}  / \textbf{63.9}  /\textbf{47.4 }  &\cellcolor{gray!25}\textbf{25.9}  / \textbf{48.5} / \textbf{61.4} \\
    \bottomrule
    \end{tabular}}
    \end{spacing}
    \vspace{-0.1cm}
    \caption{Comparison with denoised methods on COCO dataset based on the 12-epoch training schedule and 300 object queries.}
    \vspace{0.3cm}
    \label{tab:sap-dn-detr}
\end{table*}%




==> tabel1.tex <==



\begin{table*}[htbp]
  \centering
  \setlength \tabcolsep{8pt}
    \begin{spacing}{0.9}
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{lcccccccccc}
    \toprule
    \multicolumn{1}{l}{\textbf{Method}}  & \textbf{Epochs} & \textbf{GFLOPs} & \textbf{\#Params (M)}  & \textbf{MS} & \textbf{AP}&$\textbf{AP}_{50}$&$\textbf{AP}_{75}$ & $\textbf{Ap}_S$&$\textbf{Ap}_M$&$\textbf{Ap}_{L}$ \\
    \specialrule{0.9pt}{1.6pt}{3.6pt}
    \multicolumn{8}{l}{\textit{CNN Backbone with Other Representations}} \\
    \specialrule{0.5pt}{0.8pt}{1.7pt}
    FCOS    & 36    & 177   & -     &    $\checkmark$   & 41.0 &59.8&44.1  & 26.2&44.6&52.2 \\
    Faster R-CNN    & 37    & 180   & 42    &   $\checkmark$    & 40.2&61.0&43.8  & 24.2&43.5&52.0 \\
    Faster R-CNN+    & 109   & 180   & 42     &   $\checkmark$    & 42.0 &62.1&45.5  & 26.6&45.4&53.4 \\
    Mask R-CNN    & 36    & 260   & 44      & $\checkmark$    & 41.0&61.7&44.9  &  \  - \   & \  - \   & \  - \  \\
    Cas. Mask R-CNN          & 36    & 739   & 82    & $\checkmark$    & 46.3&64.3&50.5  & \  - \   & \  - \   & \  - \ \\
    \specialrule{0.5pt}{0.8pt}{1.7pt}
    \multicolumn{8}{l}{\textit{Transformer Model as Neck}} \\
    \specialrule{0.5pt}{0.8pt}{1.7pt}
    DETR-R50   & 50   & 86    & 41     &   \ding{55}   & 34.9 & 55.5 & 36.0  & 14.4 & 37.2 & 54.5 \\
    Deformable DETR-R50  & 50    & 78    & 34    &  \ding{55}     & 39.7&60.1&42.4  & 21.2&44.3&56.0 \\
    Conditional DETR-R50  & 50   & 90    & 44    &     \ding{55}  & 40.9 & 61.8 &43.3  & 20.8&44.6&59.2 \\
    SMCA-DETR-50   & 50    & 86   & 40      &   \ding{55}   & 41.0& \,\  - \,\ & \,\  - \,\     & 21.9&44.3&59.1 \\
    SAM-DETR-w/SMCA-R50 & 50 & 100 & 58 & \ding{55}   & 41.8& 63.2 & 43.9  & 22.1&45.9&60.9 \\
    Anchor-DETR-R50    & 50    & 92.7 & 39     &   \ding{55}    & 42.1&63.1&44.9  & 22.3&46.2&60.0 \\
    DAB-DETR-R50  & 50    & 100   & 44    &   \ding{55}    & 42.6&63.2&45.6  & 21.8&46.2&61.1 \\
    \specialrule{0.5pt}{0.8pt}{1.7pt}
    \multicolumn{8}{l}{\textit{Transformer Model as Neck}} \\
    \specialrule{0.5pt}{0.8pt}{1.7pt}
    DETR-R50   & 50   & 86    & 41     &   \ding{55}   & 34.9 & 55.5 & 36.0  & 14.4 & 37.2 & 54.5 \\
    Deformable DETR-R50  & 50    & 78    & 34    &  \ding{55}     & 39.7&60.1&42.4  & 21.2&44.3&56.0 \\
    Conditional DETR-R50  & 50   & 90    & 44    &     \ding{55}  & 40.9 & 61.8 &43.3  & 20.8&44.6&59.2 \\
    SMCA-DETR-50   & 50    & 86   & 40      &   \ding{55}   & 41.0& \,\  - \,\ & \,\  - \,\     & 21.9&44.3&59.1 \\
    SAM-DETR-w/SMCA-R50 & 50 & 100 & 58 & \ding{55}   & 41.8& 63.2 & 43.9  & 22.1&45.9&60.9 \\
    Anchor-DETR-R50    & 50    & 92.7 & 39     &   \ding{55}    & 42.1&63.1&44.9  & 22.3&46.2&60.0 \\
    DAB-DETR-R50  & 50    & 100   & 44    &   \ding{55}    & 42.6&63.2&45.6  & 21.8&46.2&61.1 \\
    
    % SAP-DETR-R50 & 50 &  & -     &       &   \ding{55} & 
    \bottomrule
    \end{tabular}}
  \end{spacing}
  \caption{Comparison between Transformer necks and representative CNNs with ResNet-50 backbone on COCO 2017 val set. ``GPUs Time'' denotes the training time on our 8$\times$V100 GPUs with 32 batch size;  ``MS'' denotes to multi-scale features.}
  \label{tab:31}
\end{table*}%

==> tabel3.tex <==
\begin{table*}[ht]
\centering
  \setlength \tabcolsep{5pt}
    \begin{spacing}{0.85}
    \resizebox{0.93\linewidth}{!}{%
    \begin{tabular}{lccccccccc}
    \toprule
    Method & \#Epochs& \#Params(M) & GFLOPs& AP&AP_{\text{50}}&AP_{\text{75}} & AP_{\text{S}}&AP_{\text{M}}&AP_{\text{L}} \\
    \specialrule{0.9pt}{1.6pt}{3.6pt}
    \multicolumn{10}{l}{\textit{\textbf{3Encoder-3Decoder Transformer Neck with ResNet-50 Backbone}}} \\
    \specialrule{0.5pt}{0.8pt}{1.7pt}
    DETR-R50 & 12  & 33   & 82    &       &       &    &&&     \\
    Deformable DETR-R50& 12 & 30   & 77    &       &       &  &&&       \\
    SMCA-DETR-R50       & 12  & -  & -  & 28.2 & 47.6 & 29.1 & 13.3 & 31.1 & 39.7  \\
    Conditional DETR-R50& 12  & 40 & 82 & 28.4 & 47.1 & 29.3 & 12.8 & 31.2 & 42.2  \\
    Anchor DETR-R50     & 12  & 31 & 79 & 29.9 & 50.2 & 30.6 & 13.7 & 33.3 & 42.7  \\
    DAB-DETR-R50        & 12  & 34 & 87 & 31.3 & 50.0 & 32.5 & 14.5 & 34.3 & 45.3  \\
    SAM-DETR-w/SMCA-R50 & 12  & 41 & 89 &    34.1   &   53.8    & \textbf{35.9} & \textbf{16.5} & 37.5 & 51.0     \\
    SAP-DETR-R50 (Ours) & 12  & 36 & 88 &  \textbf{34.6}     &   \textbf{54.8}    &  35.8  &15.0&\textbf{38.1}& \textbf{53.0}   \\
    \specialrule{0.5pt}{0.8pt}{1.7pt}
    DETR-R50 & 36  & 33   & 82    &       &       &    &&&     \\
    Deformable DETR-R50& 36 & 30   & 77    &       &       &  &&&       \\
    SMCA-DETR-R50      & 36 &    &       & 36.5 & 57.5 & 38.7 & 18.7 & 39.6 & 52.4   \\
    Conditional DETR-R50& 36  & 40   & 82 & 36.8 & 57.4 & 39.0 & 17.9 & 39.9 & 54.1      \\
    Anchor DETR-R50    & 36 & 31 & 79 & 36.6 & 57.8 & 38.5 & 18.1 & 40.4 & 52.6    \\
    DAB-DETR-R50       & 36 & 34 & 87 & 39.0 & 58.6 & 41.8 & 20.0 & 42.5 & 56.0  \\
    SAM-DETR-w/SMCA-R50& 36 & 41 & 89 & \textbf{40.2} & \textbf{60.5} & \textbf{42.5} & \textbf{20.2} & \textbf{44.3} & 58.3     \\
    SAP-DETR-R50 (Ours)& 36 & 36 & 88 & 39.8 & 60.3 & 41.9 & 18.2 & 43.7 & \textbf{59.2}   \\
    \specialrule{0.9pt}{1.6pt}{3.6pt}
    \multicolumn{10}{l}{\textit{\textbf{6Encoder-6Decoder Transformer Neck with ResNet-50 Backbone}}} \\
    \specialrule{0.5pt}{0.8pt}{1.7pt}
    DETR-R50& 12  & 42   & 89    &       &       &     &&&   \\
    Deformable DETR-R50& 12 & 34   & 81    &       &       &    &&&   \\
    SMCA-DETR-R50         & 12 &  - &  -  & 32.4 & 52.3 & 34.0 & 15.5 & 34.9 & 47.7  \\
    Conditional DETR-R50  & 12 & 44 & 90  & 33.1 & 53.0 & 34.8 & 14.5 & 35.9 & 49.2 \\
    Anchor DETR-R50       & 12 & 41 & 89  & 33.7 & 54.5 & 35.1 & 15.6 & 37.3 & 49.8 \\
    DAB-DETR-R50          & 12 & 44 & 96  & 34.9 & 55.5 & 36.4 & 16.2 & 38.4 & 51.5 \\
    SAM-DETR-w/SMCA-R50   & 12 & 59 & 105 & 36.2 & \textbf{57.2} & 37.4 & 16.1 & 39.8 & 55.3    \\
    SAP-DETR-R50 (Ours)   & 12 & 47 & 104 & \textbf{36.6} & 57.0 & \textbf{38.1} & \textbf{16.6} & \textbf{40.4} & \textbf{55.8}  \\
    \specialrule{0.9pt}{1.6pt}{3.6pt}
    DETR-R50             & 36  & 42   & 89    &       &       &     &&&   \\
    Deformable DETR-R50  & 36 & 34   & 81    &       &       &    &&&   \\
    SMCA-DETR-R50        & 36 & -  & -   & 40.1 & 61.4 & 42.8 & 20.3 & 43.3 & 57.1   \\
    Conditional DETR-R50 & 36 & 44 & 90  & 40.2 & 61.0 & 42.4 & 19.9 & 43.5 & 58.8  \\
    Anchor DETR-R50      & 36 & 41 & 89  & 39.7 & 60.5 & 41.9 & 19.9 & 43.5 & 57.3 \\
    DAB-DETR-R50         & 36 & 44 & 96  &  &  &  &  &  &  \\
    SAM-DETR-w/SMCA-R50  & 36 & 59 & 105 & 40.9 & \textbf{62.2} & 43.1 & 20.1 & 44.7 & \textbf{60.7}   \\
    SAP-DETR-R50 (Ours)  & 36 & 47 & 104 & \textbf{41.1} & 61.4 & 43.1 & \textbf{20.2} & \textbf{45.6} & 60.4  \\
    % \specialrule{0.9pt}{1.6pt}{3.6pt}
    % \multicolumn{10}{l}{\textit{\textbf{6Encoder-6Decoder Transformer Neck with ResNet-50-DC5 Backbone}}} \\
    % \specialrule{0.5pt}{0.8pt}{1.7pt}
    % DETR-R50-DC5& 12  & 42   & 89    &       &       &     &&&   \\
    % Deformable DETR-R50-DC5& 12 & 34   & 81    &       &       &    &&&   \\
    % Conditional DETR-R50-DC5 &12 & 44   & 90    &       &       &   &&&   \\
    % SMCA-DETR-R50-DC5& 12 &       &       &       &       &    &&&   \\
    % SAM-DETR-w/SMCA-R50-DC5& 12& 59   & 105   &       &       &   &&&    \\
    % Anchor DETR-R50-DC5& 12 & 41   & 89    &       &       &    &&&   \\
    % DAB-DETR-R50-DC5& 12  & 44  & 96    &       &       &     &&&  \\
    % SAP-DETR-R50-DC5 (Ours)& 12 & 47   & 104   &       &       &    &&&   \\
    \specialrule{0.5pt}{0.8pt}{1.7pt}
    \end{tabular}
    }
  \end{spacing}
  \caption{Comparison between Transformer necks and representative CNNs with ResNet-50 backbone on COCO 2017 val set.}
  \label{tab:31}
\end{table*}%


==> table_mask.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet4'
\begin{table}[t]
 \vspace{0.3cm}
  \centering
  \setlength \tabcolsep{3pt}
    \begin{spacing}{1}
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{c|c|c|c|c|c|c}
    \shline
    \hline
    Mode&No Mask & Layer 0 & Layer 1 & Layer 2 & Layer 3 & Layer 4 \\
    \hline
    AP&   0   &   -0.9    &    -0.2   &   -0.1    &   +0.1    & 0 \\
    \hline
    % GFLOPs&8.54/94      &  8.07/93.6     &   8.17/93.7    &  8.26/93.8     &  8.35/93.9    & 8.45/94 \\
    GFLOPs&8.54      &  8.07     &   8.17    &  8.26     &  8.35    & 8.45 \\
    \shline
    \hline
    Mode&Layer 1,2 & Layer 1,3 & Layer 1,4 & Layer 2,3 & Layer 2,4 & Layer 3,4 \\
    \hline
    AP&    -0.6  &   \textbf{+0.2}    &   -0.4    &   +0    &   -0.4    &  +0.1\\
    \hline
    % GFLOPs&  8.03/93.6    & 8.07/93.7      &  8.12/93.7     &   8.17/93.8    &   8.21/93.8    & 8.31/93.9 \\
    GFLOPs&  8.03   & 8.07      &  8.12     &   8.17    &   8.21    & 8.31 \\
    \shline
    \hline
    \end{tabular}}
  \end{spacing}
  \caption{Ablation of mask layer. The GFLOPs of the decoder layer and the change AP relative to no mask.}
  \label{tab:mask}%
\end{table}%


==> table_movepoint.tex <==
% \begin{table}[t]
%   \centering
%   \setlength \tabcolsep{2pt}
%     \begin{spacing}{0.8}
%     \resizebox{0.95\linewidth}{!}{%
%     \begin{tabular}{c|lcccc}
%     \toprule
%     \specialrule{0pt}{0.9pt}{3pt}
%     Structure & \multicolumn{1}{l}{Comments} & AP & AP$_{\text{S}}$ & AP$_{\text{M}}$ &  AP$_{\text{L}}$\\
%     \specialrule{0pt}{0.9pt}{1.3pt}
%     \toprule
%     \multirow{3}[1]{*}{\makecell[c]{3-3 Layer \\ SAP-DETR}} & Fixed Point & 40.1 & 19.2 & 44.1 & 59.0 \\
%     % fake
%     & Offset within image & 39.8 (\textcolor{csam}{-0.3}) & 19.6 (\textcolor{red}{+0.4}) & 44.0 (\textcolor{csam}{-0.1}) & 58.0 (\textcolor{csam}{-1.0})\\
%     & Offset within grid  & \textbf{40.8} (\textcolor{red}{\textbf{+0.7}}) & \textbf{20.9} (\textcolor{red}{\textbf{+1.7}}) & \textbf{44.3} (\textcolor{red}{\textbf{+0.2}}) & \textbf{59.0} \\
%     \specialrule{1pt}{0.9pt}{1.3pt}
%     \multirow{3}[1]{*}{\makecell[c]{6-6 Layer \\ SAP-DETR}} & Fixed Point         & 41.3 & 20.0 & \textbf{45.8} & \textbf{61.5} \\
%     % fake
%     & Offset within image & 41.1 (\textcolor{csam}{-0.2}) & 20.3 (\textcolor{red}{+0.3}) & 45.2 (\textcolor{csam}{-0.6}) & 60.3 (\textcolor{csam}{-1.2})\\
%     & Offset within grid  & \textbf{42.0} (\textcolor{red}{\textbf{+0.7}}) & \textbf{21.9} (\textcolor{red}{\textbf{+1.9}}) & 45.5 (\textcolor{csam}{-0.3}) & 60.8 (\textcolor{csam}{-0.7}) \\
%      \specialrule{0pt}{2pt}{1pt}
%      \bottomrule
%     \end{tabular}}
%   \end{spacing}
%   \caption{Ablation on reference point offsets.}
%   \label{tab:effectiveness}
% \end{table}%



\begin{table}[t]
  \centering
  \setlength \tabcolsep{6pt}
    \begin{spacing}{1}
    \resizebox{0.95\linewidth}{!}{%
    \begin{tabular}{c|lcccc}
    \toprule
    \specialrule{0pt}{0.9pt}{3pt}
    Structure & \multicolumn{1}{l}{Comments} & AP & AP$_{\text{S}}$ & AP$_{\text{M}}$ &  AP$_{\text{L}}$\\
    \specialrule{0pt}{0.9pt}{1.3pt}
    \toprule
    \multirow{3}[1]{*}{\makecell[c]{3-3 Layer \\ SAP-DETR}} & \makecell[l]{Indep. box head \\ \& Shared cls. head} & 40.1 & 19.2 & 44.1 & 59.0 \\
    \specialrule{0pt}{0.5pt}{1pt}
    & \makecell[l]{Indep. box head \\ \& First Indep. cls. head} & \textbf{40.4} & \textbf{19.2} & \textbf{44.6} & \textbf{59.6} \\
    
    \specialrule{0.5pt}{0.8pt}{1.2pt}
    
    \multirow{3}[1]{*}{\makecell[c]{6-6 Layer \\ SAP-DETR}} & \makecell[l]{Indep. box head \\ \& Shared cls. head} & 41.2 & \textbf{20.0} & 45.6 & 61.2 \\
    \specialrule{0pt}{0.5pt}{1pt}
    & \makecell[l]{Indep. box head \\ \& First Indep. cls. head} & \textbf{41.3} & 19.9 & \textbf{45.8} & \textbf{61.1} \\
     \specialrule{0pt}{1.5pt}{0.8pt}
     \bottomrule
    \end{tabular}}
  \end{spacing}
  \caption{Ablation on classification head.}
  \label{tab:effectiveness}
\end{table}%


